Physics-based Scene Layout Generation from Human Motion

Creating scenes for captured motions that achieve realistic human-scene interaction is crucial for 3D animation in movies or video games. As character motion is often captured in a blue-screened studio without real furniture or objects in place, there may be a discrepancy between the planned motion and the captured one. This gives rise to the need for automatic scene layout generation to relieve the burdens of selecting and positioning furniture and objects. Previous approaches cannot avoid artifacts like penetration and floating due to the lack of physical constraints. Furthermore, some heavily rely on specific data to learn the contact affordances, restricting the generalization ability to different motions. In this work, we present a physics-based approach that simultaneously optimizes a scene layout generator and simulates a moving human in a physics simulator. To attain plausible and realistic interaction motions, our method explicitly introduces physical constraints. To automatically recover and generate the scene layout, we minimize the motion tracking errors to identify the objects that can afford interaction. We use reinforcement learning to perform a dual-optimization of both the character motion imitation controller and the scene layout generator. To facilitate the optimization, we reshape the tracking rewards and devise pose prior guidance obtained from our estimated pseudo-contact labels. We evaluate our method using motions from SAMP and PROX, and demonstrate physically plausible scene layout reconstruction compared with the previous kinematics-based method.

==> section/6-figureonly.tex <==
% \begin{figure}[b]
%     \centering
%         \includegraphics[width=0.95\linewidth]{figure/skeleton.jpg}
%     \medskip
%         \includegraphics[width=0.95\linewidth]{figure/contact_val_500.pdf}
%     \caption{Visualizations of contact frame values and pseudo contact labels. The top figure presents skeleton pose snapshots, while the bottom plot displays the estimated contact frame values from the frame value networks after 500 updates. The shadow areas represent the pseudo contact labels. The visualization demonstrates the frame value network's ability to predict approximate correct contacts at an early stage of training.}
%     \label{fig:contact_val}
% \end{figure}

\begin{figure*}[p]
    \centering
    \includegraphics[width=\textwidth]{figure/comparison_MIME.pdf}
    \caption{Qualitative comparison with MIME~\cite{yi2023mime}. The results exclusively focus on the contacting objects within the scene. Our method demonstrates enhanced physical plausibility in object placements, while MIME occasionally encounters difficulties in generating scenes with satisfactory human-scene interaction, even after employing scene refinement.}
    \label{fig:comparison_mime}
\end{figure*}


